Person-in-Context Synthesiswith Compositional Structural Space

Despite significant progress, controlled generation of complex images with interacting people remains difficult. Existing layout generation methods fall short of synthesizing realistic person instances; while pose-guided generation approaches focus on a single person and assume simple or known backgrounds. To tackle these limitations, we propose a new problem, \textbf{Persons in Context Synthesis}, which aims to synthesize diverse person instance(s) in consistent contexts, with user control over both. The context is specified by the bounding box object layout which lacks shape information, while pose of the person(s) by keypoints which are sparsely annotated. To handle the stark difference in input structures, we proposed two separate neural branches to attentively composite the respective (context/person) inputs into shared ``compositional structural space'', which encodes shape, location and appearance information for both context and person structures in a disentangled manner. This structural space is then decoded to the image space using multi-level feature modulation strategy, and learned in a self supervised manner from image collections and their corresponding inputs. Extensive experiments on two large-scale datasets (COCO-Stuff \cite{caesar2018cvpr} and Visual Genome \cite{krishna2017visual}) demonstrate that our framework outperforms state-of-the-art methods w.r.t. synthesis quality.

==> table/table_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\caption{Ablation result of FID and Inception Score at 128 resolution from COCO-Stuff dataset. Removal of any component will decrease the performance.}
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
      Method                & FID & IS \\ \midrule
Ours (No Style Embedding)    & 50.6     & 10.2$\pm$0.2       \\
Ours (No Instance Attention) & 70.9     & 7.7$\pm$0.1       \\
Ours (No Person Branch)      & 55.1      & 9.9$\pm$0.1       \\
Ours (Full Method)           & \textbf{48.7}      & \textbf{10.6$\pm$0.3}      \\ \bottomrule
\end{tabular}
\vspace{-15pt}
\label{tab:ablation_study}
\end{table}

==> table/table_diff_split.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
%\resizebox{0.5\textwidth}{!}{
\caption{The FID and Inception Score on proposed person split dataset at 128$\times$128 resolution and cropped persons at 64$\times$64 resolution from COCO-Stuff dataset.}
\begin{tabular}{@{}lcccc@{}}
\toprule
Dataset          & \multicolumn{2}{c}{Person Split} & \multicolumn{2}{c}{Person Crop} \\ \midrule
Metrics          & FID        & IS     & FID       & IS     \\ \midrule
Real Images            & 0          & 17.0$\pm$0.3          & 0         & 8.9$\pm$0.4    \\
LostGAN~\cite{sun2019image}          & 96.7      & 9.2$\pm$0.6           & 77.6     & 6.2$\pm$0.3                \\
Scene Generation~\cite{ashual2019specifying} & 101.9     & 7.4$\pm$0.3           & 78.8    & 6.0$\pm$0.1                \\
GauGAN~\cite{Park2019GauGANSI}         & -          & -                   & 94.9     & 3.8$\pm$0.1                \\
Ours             & \textbf{75.6}      & \textbf{10.4$\pm$0.3}           & \textbf{52.8}     & \textbf{6.6$\pm$0.2}                \\ \bottomrule
\end{tabular}
%}
\label{tab:person_split}
\vspace{-15pt}
\end{table}

==> table/table_quantitative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\caption{A quantitative comparison using various image generation scores on COCO-Stuff and Visual Genome dataset.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}clcccccccc@{}}
\toprule
\multicolumn{2}{c}{Dataset}                   & \multicolumn{4}{c}{COCO-Stuff}                 & \multicolumn{4}{c}{Visual Genome}      \\ \midrule
Resolution               & \multicolumn{1}{c}{Method}             & IS$\uparrow$          & FID$\downarrow$   & Acc$\uparrow$   & Diversity$\uparrow$ & IS$\uparrow$  & FID$\downarrow$   & Acc$\uparrow$   & Diversity$\uparrow$ \\ \midrule
\multirow{6}{*}{64x64}   & Real Images        & 16.3$\pm$0.4           & 0     & 55.2 & -       & 13.9$\pm$ 0.5  & 0     & 49.1 & -       \\
                         & Sg2im~\cite{johnson2018image}              & 7.3$\pm$0.1            & 86.5  & 30.0 & 0.02$\pm$0.01 & 6.3$\pm$0.2    & 65.4  & 40.3 & 0.15$\pm$0.12 \\
                         & Layout2im \cite{zhao2019image}         & 9.1$\pm$0.1            & 44.2 & \textbf{50.8} & 0.15$\pm$0.06 & \textbf{9.1$\pm$0.1}    & 39.7 & \textbf{48.1} & 0.17$\pm$0.09 \\
                         & Scene Generation~\cite{ashual2019specifying} & \textbf{10.3$\pm$0.1}           & 48.7  & 46.1  & \textbf{0.43$\pm$0.07} & -        & -   & -   & -       \\
                         & LostGAN~\cite{sun2019image}            & 9.8 $\pm$ 0.2          & \textbf{34.1}  & 41.8 & 0.35$\pm$0.09 & 8.7 $\pm$ 0.4  & \textbf{32.6} & 37.6 & \textbf{0.34$\pm$0.10} \\
                         & Ours               & 9.2$\pm$0.2          & 37.4  & 43.7 & 0.27$\pm$0.08 & 8.6$\pm$0.3  & 34.1 & 47.5 & 0.26$\pm$0.09 \\ \midrule
\multirow{4}{*}{128x128} & Real Images        & 24.2$\pm$0.9 & 0     & 55.5 & -       & 23.5$\pm$0.4  & 0     & 57.2 & -       \\
                         & Scene Generation~\cite{ashual2019specifying} & 12.5$\pm$0.3           & 59.5  & 40.2  & 0.35$\pm$0.08 & -        & -   & -   & -       \\
                         & LostGAN~\cite{sun2019image}            & \textbf{13.7$\pm$0.3}          & 49.1  & 38.2  & \textbf{0.40$\pm$0.09} & 10.7$\pm$0.2  & 46.8  & 34.6  & \textbf{0.43$\pm$0.09} \\
                         & Ours               & 11.6$\pm$0.3         & \textbf{48.6}  & \textbf{41.2} & 0.33$\pm$0.12 & \textbf{11.0 $\pm$ 0.1}       & \textbf{46.2}  & \textbf{49.1} & 0.32$\pm$0.09 \\ \midrule
\multirow{3}{*}{256x256}                  & Real Images        & 30.7$\pm$1.2           & 0     & 59.1 & -       & 31.9$\pm$1.4   & 0     & 60.6 & -       \\
                         & Scene Generation~\cite{ashual2019specifying} & 14.5$\pm$0.1           & 65.2  & 42.1  & \textbf{0.48$\pm$0.09} & -        & -   & -   & -       \\
                         & Ours               & \textbf{15.2$\pm$0.5}          & \textbf{54.9}  & \textbf{42.5}  & 0.38$\pm$0.09 & \textbf{14.1$\pm$0.4} & \textbf{49.9} & \textbf{50.9} & \textbf{0.36$\pm$0.1} \\ \bottomrule
\end{tabular}
}
\vspace{-20pt}
\label{tab:all_comparision}
\end{table*}
